Efficient Poverty Mapping using Deep Reinforcement Learning

The combination of high-resolution satellite imagery and machine learning have proven useful in many sustainability-related tasks, including poverty prediction, infrastructure measurement, and forest monitoring. However, the accuracy afforded by high-resolution imagery comes at a cost, as such imagery is extremely expensive to purchase at scale. This creates a substantial hurdle to the efficient scaling and widespread adoption of high-resolution-based approaches. To reduce acquisition costs while maintaining accuracy, we propose a reinforcement learning approach in which free low-resolution imagery is used to dynamically identify where to acquire costly high-resolution images, prior to performing a deep learning task on the high-resolution images. We apply this approach to the task of poverty prediction in Uganda, building on an earlier approach that used object detection to count objects and use these counts to predict poverty. Our approach exceeds previous performance benchmarks on this task while using 80% fewer high-resolution images. Our approach could have application in many sustainability domains that require high-resolution imagery.

==> approach.tex <==
\section{Adaptive Tile Selection}
% \vspace{-0.8em}
\label{sec:generic}
% \begin{figure*}[!h]
% \centering
%     \includegraphics[width=0.80\textwidth]{images/influence.png}
%     \caption{The proposed Bayesian influence diagram. We condition the agent on LR image to dynamically sample HR images from the subset of area covered by LR image. We train the agent so that it only samples HR images where there are objects of interest.}
%     \label{fig:influence_diagram}
% \end{figure*}

%The previous study samples HR images exhaustively with a fixed policy across the clusters to approximate the object detections accurately~\cite{ayush2020generating}. 
Due to the large acquisition cost of HR images, it is non-trivial and expensive to deploy models based on HR imagery at scale. For this reason, we propose an efficient tile selection framework to capture relevant fine level information such as classwise object counts for downstream tasks. We represent the HR image covering a spatial cluster $i$ centered at $c_{i}=(c_{i}^{lat},c_{i}^{lon})$ as $\mathcal{H}_{i} \in R^{W \times H \times B}$ where $W$, $H$ and $B$ represent height width and number of bands. Additionally, we represent the LR image of the same spatial cluster $i$ as $\mathcal{L}_{i} \in R^{W/D, H/D, B}$ where $D$ represents a scalar for the number of pixels in width and height. For example, in the case of Sentinel-2 (10 m GSD), we have $D=30$ times smaller number of pixels than the high-resolution DigitalGlobe images (0.3m GSD).
With an adaptive approach, our task is to acquire only small subset of $\mathcal{H}_{i}$ conditionally on $\mathcal{L}_{i}$ while not hurting the performance in our downstream tasks that uses object counts from the cluster $i$.
% We perform an initial search space optimization on \emph{very large} images with around 34,000 pixels in each dimension. At the end of the search, we find an initial set of tiles where it may be beneficial to zoom-in and acquire HR images for object detection. 
This adaptive method is formulated as a two-step episodic Markov Decision Process (MDP), similar to~\cite{uzkent2020efficient}. In the first step, we adaptively sample HR tiles and in the second step, we run them through a pre-trained detector.
% In the diagram, we represent random variables with a circle, actions with a square/rectangle, and utilities with a diamond.

\textbf{Adaptive Selection.}
The first module of our framework finds HR tiles to sample/acquire, conditioned on the low spatial resolution image covering a cluster. 
%This is achieved by applying the proposed generic influence diagram as shown in Fig.~\ref{fig:influence_diagram}. 
In this direction, a cluster-level HR image $\mathcal{H}_{i} = (H_{i}^{1}, H_{i}^{2},\dotsc, H_{i}^{T})$ is divided into equal-size non-overlapping tiles, where $T$ is the number of tiles. In this set up, we model $\mathcal{H}_{i}$ as a latent variable as it is not directly observed and it is inferred from the random variable $\mathcal{L}_{i}$. We associate each tile, $H_{i}^{j}$, of $\mathcal{H}_{i}$ with an $L$-dimensional classwise object counts feature represented as  
$\mathbf{v}_i=\{\mathbf{v}^1_i, \dotsc, \mathbf{v}^{T}_i\}$. We then model the policy network to only choose tiles where there is desirable number of object counts as:  \textbf{Acquire} $H_{i}^{j}$ if $||\mathbf{v}^j_i||_{1} > P$ where $P$ is determined by the policy network that uses a reward function characterized by the user. Similar to $\mathcal{H}_{i}$, we decompose the random variable $\mathcal{L}_{i}$ as $\mathcal{L}_{i} = (l_{i}^{1}, l_{i}^{2},\dotsc, l_{i}^{T})$ where $l_{i}^{j}$ represents the lower spatial resolution version (from Sentinel-2) of $H_{i}^{j}$. 
\se{this is confusing}

\textbf{Modeling the Policy Network's Input and Output.} In a simple scenario, we can take a single binary action for each $H_{i}^{j}$ whether to acquire it or not conditioned on $l_{i}^{j}$. However, we believe that choosing multiple actions representing different disjoint subtiles of tile $H_{i}^{j}$ can help us avoid sampling areas of tile $H_{i}^{j}$ where there are no objects of interest. In another setup, we can use a large $T$ to have smaller tiles and take a single action to sample tile $H_{i}^{j}$ or not. However, this  introduces run-time complexity since we need to run the policy network more number of times to cover a cluster. For these reasons, we divide tile $H_{i}^{j}$ into $S$ number of disjoint subtiles as $H_{i}^{j}=(h_{i}^{j,1},h_{i}^{j,2},...,h_{i}^{j,S})$.
In the first step of the MDP, the agent observes $l_{i}^{j}$ and outputs a binary action array, $\mathbf{a}_{i}^{j} \in \{0,1\}^{S}$, where $a_{i}^{j,k} = 1$ represents acquisition of the HR version of the $k$-th subtile of $H_{i}^{j}$ \emph{i.e.} $h_{i}^{j,k}$. The subtile sampling policy, parameterized by $\theta_{p}$, is formulated as
\begin{equation}
    \pi(\mathbf{a}_{i}^{j} | l_{i}^{j};\theta_{p}) = p(\mathbf{a}_{i}^{j}|l_{i}^{j};\theta_{p})
\label{eq:policy_cpnet}
\end{equation}
where $\pi(l_{i}^{j};\theta_{p})$ is a function mapping the observed LR image to a probability distribution over subtile sampling actions $\mathbf{a}_i^j$. The joint probability distribution over the random variables $l_{i}^{j}$, $\mathbf{v}_{i}^{j}$, $H_{i}^{j}$, and action $\mathbf{a}_{i}^{j}$, can be written as 
% $p(H_{i}^{j}, l_{i}^{j}, \mathbf{v}_{i}^{j}, \mathbf{a}_{i}^{j}) = p(H_{i}^{j})\, p(\mathbf{v}_{i}^{j}|H_{i}^{j})\, p(l_{i}^{j}|H_{i}^{j})\, p(\mathbf{a}_{i}^{j}|l_{i}^{j};\theta_{p})$.

\begin{equation}
    p(H_{i}^{j}, l_{i}^{j}, \mathbf{v}_{i}^{j}, \mathbf{a}_{i}^{j}) = p(H_{i}^{j})\, p(\mathbf{v}_{i}^{j}|H_{i}^{j})\, p(l_{i}^{j}|H_{i}^{j})\, p(\mathbf{a}_{i}^{j}|l_{i}^{j};\theta_{p})
\label{eq:joint_distribution_cpnet}
\end{equation} 

\textbf{Object Detection.} In the second step of the MDP, the agent runs the object detection on the selected HR subtiles. Conditioned on $\mathbf{a}_{i}^{j}$, it observes HR subtiles if necessary and produces $\mathbf{\hat{v}}_{i}^j$, a $L$-dimensional classwise object counts vector. We find the object counts with our adaptive framework using a pre-trained object detector $f_d$ (parameterized by $\theta_d$) as:
\begin{equation}
\hat{\mathbf{v}}_{i}^{j,k} = \left\{ \begin{array}{ll} f_{d}(h_{i}^{j,k}) \quad \text{if} \quad a_{i}^{j,k}=1 \\ \mathbf{0} \quad \text{else} \end{array} \right.
\end{equation}
Then, we compute the tile level object counts as $\mathbf{\hat{v}}_{i}^j = \sum_{k=1}^{S} \mathbf{\hat{v}}_{i}^{j,k}$. Finally,  we define our overall cost function $J$ as:
\begin{equation}
\max_{\theta_{p}} J(\theta_{p}, \theta_{d}) = \mathbb{E}_p[R(\mathbf{a}_i^j, {\mathbf{\hat{v}}_i^j}, \mathbf{v}_i^j)],
\label{Eq:Cost_Function}
\end{equation}
where the reward depends on $\mathbf{a}_{i}^{j}$, $\mathbf{\hat{v}}_i^j$, $\mathbf{v}_i^j$. 
% The reward penalizes the agent for selecting a large number of HR tiles (e.g., based on the norm of $a_i^j$) and includes a performance metric evaluating the accuracy of sampled features, $\hat{\mathbf{m}_i}$, given the true label $\mathbf{m}_i$ (e.g.,  norm of difference of $\hat{\mathbf{m}_i}$ and $\mathbf{m}_i$). 
Our goal is to learn the parameters $\theta_{p}$ given a pre-trained object detector $\theta_d$ to maximize the objective being a function of the reward function. We detail the reward function in the next section.%~\ref{sect:reward_function}.

\section{Modeling and Optimization of the Policy Network}
\label{sec:reward_function}
% \vspace{-0.8em}
\textbf{Modeling the Policy Network.} In the previous section, in high level we formulated the task of efficient HR subtile selection as a two step episodic MDP. In this section, we model how to learn the policy distribution for subtile sampling. In this study, we have $T=1156$ number of tiles as we have a 34$\times$34 grid of images. In this case, each tile consists of 1000$\times$1000 pixels. As mentioned in the previous section, we divide each tile into S=4 subtiles of 250$\times$250 pixels each (higher values of $S$ led to unstable training with higher variance and less sparse selections).
% In the first step of the two step MDP, the policy network, $f_{p}$, \emph{output the probabilities for all the actions at once} after observing $l_{i}^{j}$. An alternative approach could be in the form a sequential decision framework where each action depends on the action on the previous HR tile.
% An alternative approach could be in the form of a framework where $a_{i}^{j}^{i,j}$ is conditioned on $a_{i}^{j}^{1:i-1,1:j-1}$.
% The proposed concept of \emph{outputting all the actions at once} provides a more efficient decision making process.
In this study, similar to~\cite{uzkent2020efficient} we model the action likelihood function of the policy network, $f_{p}$, using the product of bernoulli distributions as:
\begin{align}
  \pi(\mathbf{a}_{i}^{j}|l_{i}^{j}; \theta_{p}) &= \prod_{k=1}^{S} (s_{i}^{j,k})^{a_i^{j,k}} (1- s_{i}^{j,k})^{(1-a_{i}^{j,k})} 
%   \\
%   \pi_{f}(a_{f}|l_{i}^{j}^{i}; \theta_{p}^{f}) &= \prod_{j=1}^{P_f} (s_{f}^{j})^{a_f^i} (1- s_{f}^{j})^{(1-a_{f}^{j})}
\label{eq:action_likelihood}
\end{align}
%where $s_{i}^{j}$ is the prediction vector formulated as
\begin{align}
    s_{i}^{j} &= f_{p}(l_{i}^{j};\theta_{p}) 
    % \\
    % s_{f} &= f_{p}^{f}(l_{i}^{j}^{i};\theta_{p}^{f}).
\label{eq:policy_network}
\end{align}
We use a sigmoid function to transform logits to probabilistic values, $s_{i}^{j,k} \in [0,1]$.

% The next set of actions for the coarse level search, $a_{d}$, is chosen by the coarse and fine level object detectors using the LR tile $l_{i}^{j}^{i}$ or the sampled HR tile $x_{H}^{i}$. For the fine level search, the actions, $a_{d}$, are chosen using the LR subtile $l_{i}^{j}^{i}$ or the sampled HR subtile $x_{h}^{i}$.

% \begin{wrapfigure}{r}{0.45\textwidth}
% \begin{minipage}{0.5\textwidth}
% \vspace{-0.55cm}
% \begin{algorithm}[H]
% \algsetup{linenosize=\small}
% \scriptsize
% \hline
% \vspace{0.3em}
% \SetAlgoLined
% \KwIn{($\mathcal{L}_{i}$, $\mathcal{H}_{i}$)\quad 
% $i=\{1, 2, ..., N\}$ \\}
% \For{$j\gets 1\:to\:T$}{
%     $s_{i}^{j} \gets f_{p}(l_{i}^{j};\theta_{p})$ \\
%     $s_{i}^{j} \gets \alpha + (1-s_{i}^{j})(1-\alpha)$ \\
%     $\mathbf{a}_{i}^{j} \sim \pi(\mathbf{a}_{i}^{j}|s_{i}^{j})$ \\
%     \BlankLine
%     \For{$k\gets 1\:to\:S$}{
%     $\mathbf{\hat{v}}_{i}^{j,k} = f_{d}(h_{i}^{j,k})\bigodot\:\mathbf{a}_{i}^{j,k}$ \\
%     }
%     $\mathbf{\hat{v}}_i^j = \sum_{k=1}^S \mathbf{\hat{v}}_i^{j,k}$
%     \BlankLine
%     \textbf{Evaluate Reward} $R(\mathbf{a}_{i}^{j}, \mathbf{\hat{v}}_{i}^{j}, \mathbf{v}_{i}^{j})$ \\
%     \BlankLine
%     $\theta_{p} \gets \theta_{p} + \nabla{\theta_{p}}$
% }
% \hline
% \vspace{0.2em}
% \caption{Pseudo-code for the Proposed Adaptive Algorithm. $T$ and $S$ represent the number of tiles and subtiles.}
% \label{alg:tileDrop_Algorithm}
% \end{algorithm}
% \end{minipage}
% \end{wrapfigure}
\textbf{Optimization of the Policy Network.} 
Next we detail optimization procedure for the policy network. Previously defined objective function as shown in Eq.~\ref{Eq:Cost_Function} is not differentiable w.r.t the policy network parameters, $\theta_{p}$. This is because we discretize continuous action probabilities from the policy network to perform binary action of acquiring or not acquiring a subtile.
To overcome this, we use Policy Gradient~\cite{sutton2018reinforcement}. Our final objective function as shown below includes the reward function as well as action likelihood distribution which can be differentiated w.r.t $\theta_p$.
\begin{equation}
\nabla_{\theta_{p}}J &= \mathbb{E}\left[ R(\mathbf{a}_{i}^{j}, \mathbf{\hat{v}}_{i}^{j}, \mathbf{v}_i^{j})\nabla_{\theta_{p}} \log \pi_{\theta_{p}}(\mathbf{a}_{i}^{j}|l_{i}^{j}) \right],
\label{eq:policy_gradient_coarse} 
% \\
% \nabla_{\theta_{p}^{f}}J_f &= \mathbb{E}\left[ R_f(a_{f}, a_{d}, Y_{i})\nabla_{\theta_{p}^{f}} \log \pi_{\theta_{p}^{f}}(a_{f}|l_{i}^{j}^{i}) \right].
% \label{eq:policy_gradient_fine}
\end{equation}
% Because the actions are discrete, we cannot use the reparameterization trick to optimize the objective w.r.t. $\theta_{p}$. 
% To optimize the parameters $\theta_{p}$ of $f_{p}^c$, we need to use model-free reinforcement learning algorithms such as Q-learning~\cite{Watkins92q-learning} and policy gradient~\cite{sutton2018reinforcement}. P
% Policy gradient is more suitable in our scenario since the number of unique actions the policy network can choose is $2^{P}$ and increases exponentially with $P$. 
% Finally, we use the \textit{REINFORCE} method~\cite{sutton2018reinforcement} to optimize the objective w.r.t. policy network parameters as:
Our objective function relies on mini-batch Monte-Carlo sampling to approximate the expectation. Especially, in scenarios where we can not afford large mini-batches, we can have highly oscillating expectations which results in large variance. As this can de-stabilize the optimization, we use the self-critical baseline~\cite{rennie2017self}, $A$, to reduce the variance.
\begin{equation}
\nabla_{\theta_{p}}J = \mathbb{E}\left[ A \sum_{k=1}^{S} \nabla_{\theta_{p}}\log(s_{i}^{j,k}\mathbf{a}_{i}^{j,k}+(1-s_{i}^{j,k})(1-\mathbf{a}_{i}^{j,k})) \right]
\end{equation}
\begin{equation}
    A(\mathbf{a}_i^j, \mathbf{a'}_i^j) = R(\mathbf{a}_i^j, \mathbf{\hat{v}}_i^j, \mathbf{v}_i^j) - R(\mathbf{a'}_i^j, \mathbf{\hat{v}'}_i^j, \mathbf{v}_i^j)
\end{equation}
% Since this can lead to an unstable training process~\cite{wu2018blockdrop}, we replace $R(a_{i}^{j}, \hat{\mathbf{m}_i}, \mathbf{m}_i)$ in Eq.~\ref{eq:policy_gradient_coarse} with the advantage function to reduce the variance:

where $\mathbf{a'}_{i}^{j}$ represents the baseline action vector. To get $\mathbf{a'}_{i}^{j}$, we use the most likely action vector proposed by the policy network: \textit{i.e.}, $a'_{i}^{j,k}=1$ if $s_{i}^{j,k}>0.5$ and $a'_{i}^{j,k}=0$ otherwise. 
% The object detector, $f_{d}$, then observes $h_{i}^{j,n}$, and outputs the predicted bounding boxes $\hat{\mathbf{m}}'$. The advantage function assigns the policy network \emph{a positive value} only when the action vector sampled from Eq.~\ref{eq:action_likelihood} produces higher reward than the action vector with maximum likelihood, which is known as a self-critical baseline~\cite{rennie2017self}.
% Similarly to the coarse level search, we introduce the advantage function to the \emph{fine level search} module and do not show it in this section for simplicity.
Finally, in this study we use temperature scaling~\cite{sutton2018reinforcement} to adjust exploration/exploitation trade-off during optimization time as
\begin{equation}
s_{i}^{j,k} = \alpha s_{i}^{j,k} + (1-\alpha)(1-s_{i}^{j,k}).
\end{equation}
Setting $\alpha$ to a large value results in sampling from the learned policy whereas the small values lead to sampling from random policy.

\textbf{Modeling the Reward Function.}
% \label{sec:reward_function}

\se{this part should go earlier}
The proposed framework uses the policy gradient reinforcement learning algorithm to learn the parameters of the policy network $f_p$, adjusting weights $\theta_p$ to increase the expected reward value. Thus, it is crucial to design a reward function reflecting the desired characteristics of an efficient subtile selection method from a cluster representing a large area. The desired outcome from our adaptive strategy is to reduce the \emph{image acquisition cost} drastically by sampling smaller subset of tiles. Taking this into account, we design a dual reward function that encourages dropping as many subtiles as possible while successfully approximating the classwise object counts. We define $R$ as follows:
% \begin{equation}
%     R = R_{acc}(\mathbf{\hat{v}}_i^j, \mathbf{v}_i^j) + R_{cost}(\mathbf{a}_{i}^{j})
%     \text{ where }
% % \end{equation}
% % \begin{equation}
%     R_{acc} = -||\mathbf{v}_i^j - \hat{\mathbf{v}}_i^j||_1
%     % \label{eq:reward_function_acc}
%     % \text{ and } 
%     \\
% % \end{equation}
% % \begin{equation}
%     R_{cost} = \lambda(1 - |\mathbf{a}_{i}^{j}|_1 / S)
%     \label{eq:tradeoff}
% \end{equation}

\begin{equation}
R = R_{acc}(\mathbf{\hat{v}}_i^j, \mathbf{v}_i^j) + R_{cost}(\mathbf{a}_{i}^{j}) 
\end{equation}
\begin{equation}
R_{acc} = -||\mathbf{v}_i^j - \hat{\mathbf{v}}_i^j||_1
\end{equation}
\begin{equation}
R_{cost} = \lambda(1 - ||\mathbf{a}_{i}^{j}||_1 / S)
\label{eq:tradeoff}
\end{equation}
where $R_{acc}$ is object counts approximation accuracy and $R_{cost}$ represents the image acquisition cost with $\lambda$ as its coefficient. The $R_{acc}$ term encourages acquiring a subtile when the counts difference between the object counts from fixed HR subtile sampling policy and the adaptive policy is positive. 
% The difference is then scaled with the number of objects in the tile, $N_{i}$, to prioritize zooming-in to regions where \emph{there are more objects}. $\beta$, on the other hand, prioritizes using LR images when the recall values from coarse and fine detector are similar. Note that since our priority is to \emph{minimize the ratio of false negatives}, we only use Recall and do not consider \emph{Precision} in $R_{acc}$. 
We increase the reward \emph{linearly} with the smaller number of acquired subtiles for the cost component. See appendix for the pseudocode and implementation details.

==> broader_impact.tex <==

\section*{Ethics Statement}

% authors should discuss \\
% a) who may benefit from this research \\
% b) who may be put at disadvantage from this research \\
% c) what are the consequences of failure of the system \\
% d) whether the task/method leverages biases in the data


A range of organizations, from governments to non-governmental organizations to private sector enterprise, depend on accurate local-level information of economic well-being of populations for their decision-making.  Such information is expensive to collect using traditional ground-based survey operations, and as a result it rarely gets collected:  \cite{yeh2020using} calculate that for most countries in Africa, at least five years pass between nationally representative household livelihood surveys, and the number of villages covered in these surveys is incredibly small relative to the population size.  The result is an environment of data scarcity in which governments and NGOs have difficulty identifying those most in need of assistance or measuring the impact of the assistance they do deliver. 

Our approach offers an accurate, inexpensive, and scalable method for plugging this data gap. It uses only anonmyized public data in training, and these data are thought to be a true random and unbiased sample of the population (this is the explict goal of the LSMS survey team).  Thus our approach should deliver unbiased estimates of local-level well-being, and does so without having to use any individually-identifying information.

One possible concern of our approach is that better information on where the poor are could lead to them being denied certain services due to their (now-known) low income levels. We believe that this is unlikely for multiple reasons.  First, the poor are already severely underserved by private markets in much of the developing world, with (e.g.) access to bank loans among the poor typically in the low single digits \cite{suri2016long}. For these populations, better data on their location and livelihoods is expected to improve rather than diminish access to private sector services. Similarly, due to lack of data, governments have difficulty targeting existing anti-poverty programs, meaning that resources that should be going to poorer populations sometimes flow to wealthier populations; for governments that do target, ground-based survey efforts regularly cost tens of millions of dollars \cite{banerjee2019universal}.  More accurate data on the location and poverty levels of populations should increase rather than decrease resources flowing to vulnerable populations.  

==> introduction2.tex <==
\section{Introduction}
Accurate measurements of poverty and related human livelihood outcomes critically shape the decisions of governments and humanitarian organizations around the world, and the eradication of poverty remains the first of the United Nations Sustainable Development Goals \cite{assembly2015sustainable}. However, reliable local-level measurements of economic well-being are rare in many parts of the developing world.  Such measurements are typically made with household surveys, which are expensive and time consuming to conduct across broad geographies, and as a result such surveys are conducted infrequently and on limited numbers of households.  
\burak{First two paragraphs are the same as IJCAI. Needs some change.}

To address this problem, alternate strategies have used passively-collected data from non-traditional sources to shed light on local-level economic outcomes.   %Such work has shown promise in measuring certain indicators of economic livelihoods at local level. 
For instance, \cite{blumenstock2015predicting} show how features extracted from cell phone data can be used to predict asset wealth in Rwanda, and \cite{sheehan2019predicting} show how applying NLP techniques to Wikipedia articles can be used to predict asset wealth in multiple developing countries, and \cite{yeh2020using,jean2016combining,ayush2020generating} show how daytime and nighttime satellite imagery can combined to measures asset wealth across multiple African countries. %\cite{jean2016combining} show how a transfer learning approach that uses coarse information from nighttime satellite images to extract features from daytime high resolution imagery can also predict asset wealth variation across multiple African countries. 

When combined with machine learning, satellite imagery has proven more broadly useful for a range of sustainability-related tasks, owing in large part to their broad temporal and spatial coverage.
%Among these data resources, satellite images have been commonly used for a variety of tasks~\cite{zhong2017satcnn,paisitkriangkrai2016semantic,cheang2017using} including poverty prediction~\cite{jean2016combining,engstrom2017poverty,xie2016transfer} as they are becoming widely available across the world. Together with their availability at global scale, they offer high dimensional information that can be successfully analyzed with modern deep learning techniques. 
Such imagery are captured with a range of sensors that typically trade off spatial/temporal resolution and acquisition cost. Publicly available low spatial resolution images offer high level information that has been successfully applied to a variety of tasks~\cite{yeh2020using,helber2019eurosat}. On the other hand, high spatial resolution satellite images offer great amount of interpretable low level information, e.g. the number and location of objects, which is not possible to extract with low resolution counterparts. Such information has proven useful across a variety of sustainability domains, including poverty prediction~\cite{jean2016combining,ayush2020generating,engstrom2017poverty} infrastructure measurement~\cite{cadamuro2018assigning}, forest and water quality monitoring~\cite{fisher2018impact}, and the mapping of informal settlements~\cite{mahabir2018critical}. %By extracting such low level statistics, we can find out their correlation with local-level consumption expenditure as recently proposed by~\cite{ayush2020generating}. 
However, one major downside of using high resolution images is that they are financially costly, preventing the deployment of highly accurate and interpretable models at scale. 

To address this cost/accuracy trade-off, we propose a reinforcement learning approach that uses coarse, freely-available public imagery to dynamically identify when and where to acquire costly high resolution images, prior to conducting a deep learning task like object detection.  We apply our approach in the domain of poverty prediction, and show how our approach can substantially reduce the cost of previous methods that used deep learning on high resolution images to predict poverty~\cite{ayush2020generating} while maintaining or even improving their accuracy. In our study country of Uganda, we show how our approach can reduce the number of high resolution images needed by 80\%, in turn reducing the cost of making a country-wide poverty map using this approach by \$2.9 million. 
%In high level, we train an agent using \emph{reinforcement learning} to process publicly available low resolution images, i.e. Sentinel-2, to only acquire high resolution imagery when necessary. Such cost-aware approach minimizes the use of high resolution images which is critical in running at scale. Our experiments show that we can approximate the accuracy of the object counts based model proposed by~\cite{ayush2020generating} while reducing the use of high resolution images by $80\%$. More specifically, considering an area roughly equal to the size of the country of Uganda, it would cost about 760,000 dollars~\footnote{http://www.landinfo.com/satellite-imagery-pricing.html} to acquire high resolution images with a ground sampling distance of $\sim0.5$m. Our adaptive approach would reduce this number to only 152,000 dollars.

% These existing approaches to using non-traditional data are promising, given that they are in principle both less expensive and more scalable than traditional ground-based approaches, but they face two main challenges that inhibit their broader adoption by policymakers. The first is the outcome being measured.  While measures of asset ownership are thought to be relevant metrics for understanding longer-run household well-being \cite{filmer2001estimating}, official measurement of poverty requires data on consumption expenditure (i.e. the value of all goods consumed by a household over a given period), and existing methods have either not been used to predict consumption data or perform much more poorly when predicting consumption than when predicting other livelihood indicators such as asset wealth \cite{jean2016combining}.  Second, interpretability of model predictions is key for whether policymakers will adopt machine-learning based approaches to livelihoods measurement, and current approaches attempt to maximize predictive performance rather than interpretability. This tradeoff, central to many problems at the interface of machine learning and policy \cite{murdoch2019definitions}, has been recently addressed by \cite{ayush2020generating} who demonstrate an interpretable computational framework for predicting local-level consumption expenditure using object detection on high resolution (30cm) daytime satellite imagery.  

% They focus on Uganda, a country with existing high-quality ground data on consumption where performance benchmark are available, and apply a  trained satellite imagery object detector to high resolution images taken over hundreds of villages across Uganda that were measured in an existing georeferenced household survey, and use extracted counts of detected objects as features in a final prediction of consumption expenditure. However, the satellite images representing a village are on the order of several thousands of pixels (34000) in each dimension. These large images enable higher detection accuracy, especially for smaller objects relative to the field of view \cite{redmon2017yolov2}, but they require additional computation, time, and/or financial resources to process. Additionally, in realistic remote sensing applications, these high spatial resolution satellite images (e.g.$<$1m/px) are financially costly to acquire, compared to publicly available low spatial resolution satellite images (e.g. 10m/px)~\cite{drusch2012sentinel2}. Therefore, it is desirable to build a system that minimizes dependency on large images to reduce the costs of analyzing satellite images for computer vision tasks including image recognition~\cite{sheehan2018learning,uzkent2019learning}, object detection~\cite{lam2018xview,chen2014vehicle}, object tracking~\cite{uzkent2016real,uzkent2014feature}, and poverty mapping~\cite{sheehan2019predicting}.

% Directly applying existing state-of-the-art convolutional detectors on large images not only increases processing time but also the memory required to store large feature maps~\cite{lampert2008beyond,wojek2008sliding}. The traditional \textit{sliding window} approach mitigates the memory requirement by ``sliding'' the convolutional detector over crops of the image until the full image has been processed. However, the processing time of this technique increases quadratically with respect to side-length of the image, and it may have lower accuracy because the detector is unable to ``see'' the whole image at once.

% To describe our approach at a high level, we train an agent using \emph{reinforcement learning} to explicitly maximize information capture while minimizing the amount of HR images. It first processes a low resolution (LR) image, learning the global image context, then selectively requests certain HR patches that it deems necessary for object detections. Importantly, the agent is not given the HR image, thus limiting potential acquisition costs for the HR image to only the patches that it selects.

% We then apply a trained object detector to selected high resolution images for the villages across Uganda, and use extracted counts of detected objects as features in a final prediction of consumption expenditure. We show that our approach maintains high performance by using HR images only about 20\% of the time compared to \cite{ayush2020generating} that use all the HR images.
 
% \david{great intro, but there seems a disconnect b/w abstract that discusses value of reducing \# of high res images, and the intro, which doesn't mention it at all. maybe a sentence at the end here to summarize that we also show it can be done efficiently by selecting which areas to use high res images}



